Inferring Relational Potentials in Interacting Systems

Systems consisting of interacting agents are prevalent in the world, ranging from dynamical systems in physics to complex biological networks. To build systems which can interact robustly in the real world, it is thus important to be able to infer the precise interactions governing such systems. Existing approaches typically discover such interactions by explicitly modeling the feed-forward dynamics of the trajectories. In this work, we propose Neural Interaction Inference with Potentials (NIIP) as an alternative approach to discover such interactions that enables greater flexibility in trajectory modeling: it discovers a set of relational potentials, represented as energy functions, which when minimized reconstruct the original trajectory. NIIP assigns low energy to the subset of trajectories which respect the relational constraints observed. We illustrate that with these representations NIIP displays unique capabilities in test-time. First, it allows trajectory manipulation, such as interchanging interaction types across separately trained models, as well as trajectory forecasting. Additionally, it allows adding external hand-crafted potentials at test-time. Finally, NIIP enables the detection of out-of-distribution samples and anomalies without explicit training. Website: https://energy-based-model.github.io/interaction-potentials.

==> graphics/figure-method-algo.tex <==
\begin{figure}[t]
 \begin{minipage}[b]{0.62\textwidth}
    \centering
  \includegraphics[trim={10 470 680 0}, width=\textwidth]{figs/method.pdf}
    \captionof{figure}{\small \textbf{Architecture and methodology of our approach.} In the left, $\text{Enc}_{\theta}$ observes a portion of the input trajectory $\V{x}$ and encodes them into potentials, in the form of latent vectors $\V{z}_{ij,l}$. In the right, a set of energy functions parametrized as GNNs are conditioned by $\V{z}_{ij,l}$ at the edge level. We initialize a trajectory $\V{x}[0]$ as uniform noise and the ground-truth initial conditions $\V{x}^0$, and update it by minimizing the constrained energy functions. We sample by means of Langevin Dynamics. We supervise the reconstructed trajectories with an MSE objective with respect to the ground-truth.}
    \label{fig:method}
  \end{minipage}
  \hfill
  \scalebox{0.7}{
  \begin{minipage}[b]{0.5\textwidth}
%   \vspace{-20pt}
  \centering
\begin{algorithm}[H]
\small
\begin{algorithmic}
    \STATE \textbf{Input:} Full trajectories $\V{x}$, Observed trajectories $\V{x}^\text{obs}$, Initial conditions $\V{x}^0$, step size $\lambda$, number of gradient steps $M$, encoder $\text{Enc}_\theta$, energy functions $E_\theta^{ij,l}$
    \WHILE{not converged}
    \STATE $\V{x}_i \sim p_D$
    \STATE \emph{$\triangleright$ Encode components $\V{z}_{ij,l}$ from $\V{x}^\text{obs}$}
    \STATE $\{\V{z}\} \gets \text{Enc}_\theta(\V{x}^\text{obs})$
    \STATE \emph{$\triangleright$ Optimize sample  $\V{x}_i^0$ via gradient descent:}
    \STATE $\V{x}^0_i \sim \mathcal{U}(0, 1)$ 
    \FOR{gradient step $n = 1$ to $N$}
    \STATE $\Tilde{\V{x}}^m \gets   \Tilde{\V{x}}^{m-1}$
    \STATE $\quad \quad -\frac{\lambda}{2}\nabla_{\V{x}}\sum_{ij,l}{E_\theta^{ij,l}(\Tilde{\V{x}}[m-1];\V{z}_{ij,l})} $
    \ENDFOR
    \STATE \emph{$\triangleright$ Optimize objective $\mathcal{L}_{\text{MSE}}$ wrt $\theta$:} 
    \STATE $\Delta \theta \gets \nabla_\theta \|\Tilde{\V{x}}[m] - \V{x}\|^2 $
    \STATE Update $\theta$ based on $\Delta \theta$ using optimizer 
    \ENDWHILE
  \end{algorithmic}
%   \vspace{-15pt}
 \end{algorithm}
 
 \vspace{-15pt}
      \captionsetup{font=large}
      \captionof{algorithm}{\large \textbf{Training Algorithm.} \model is trained to infer a set of potentials, represented as energy functions, using a trajectory reconstruction objective. A set of latents $\{\vz\}$ is inferred from the beginning of a trajectory $\V{x}^\text{obs}$, and define different energy functions. A trajectory is optimized w.r.t. to energy functions and supervised with the full trajectory $\V{x}$. }\label{algo}
    \end{minipage}
  }  
  \end{figure}

==> graphics/table-acc.tex <==
% \begin{wrapfigure}{r}{.45\textwidth}
% \small
\begin{figure}

% \vspace{-5pt}
\centering
\begin{tabular}{l c c}
\toprule
\textbf{Model} & \textbf{Springs} & \textbf{Charged}  \\\midrule
& \multicolumn{2}{c}{5 objects}\\[0.1em]
Corr. (path)  & $52.4${\tiny$\pm$0.0} & $55.8${\tiny$\pm$0.0}\\
Corr. (LSTM) & $52.7${\tiny$\pm$0.9} & $54.2${\tiny$\pm$2.0} \\
NRI (sim.) & $\mathbf{99.8}${\tiny$\pm$0.0} & $59.6${\tiny$\pm$0.8}\\
NRI (learned) & $\mathbf{99.9}${\tiny$\pm$0.0} & $\mathbf{82.1}${\tiny$\pm$0.6} \\
\midrule
\model (linear dec.) & $97.4${\tiny$\pm$0.01} & $69.4${\tiny$\pm$1.0}\\
\bottomrule
\end{tabular}
\captionof{table}{\small \textbf{Accuracy (in $\%$) of true interaction recovery}. We train a linear decoder to predict edge types from potentials. Without supervision \model learns meaningful representations that can often recover true interactions. Corr. indicates evaluation by means of the matrix of correlations between feature vectors.}\label{tab:edge_acc} %\vspace{-15pt}
\end{figure}


==> graphics/table-nba-horizons.tex <==
% \begin{table*}[t!]
\begin{wraptable}{r}{0.6\textwidth}
\small
\centering
% \vspace{5.5em}
\vspace{-3em}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{\textbf{NBA SportsVU}}\\ \midrule
Prediction steps & 1 & 10 & 20 \\ \midrule
Static & 2.13e-4 & 3.04e-3 & 1.07e-2 \\
S-LSTM & - & - & - \\
D-LSTM & - & - & - \\
LSTM (joint) & 8.07e-5 & 1.42e-3 & 5.31e-3 \\
{Cond. GNN} & {1.71e-4} & {1.12e-3} & {3.11e-3} \\                        
NCI (Ours)  & \textbf{1.27e-5} & \textbf{3.46e-4} & \textbf{1.86e-3}\\
\midrule
& \multicolumn{3}{c}{\textbf{JPL Horizons}}\\ \midrule
% Prediction steps & 1 & 10 & 20 \\ \midrule
Static & - & - & - \\
LSTM (joint) & - & - & - \\
{Cond. GNN} & - & - & - \\  %                   
NCI (Ours)  & \textbf{-} & \textbf{-} & \textbf{-}\\ 
\bottomrule
\end{tabular}
\caption{\small Mean squared error (MSE) in predicting future states for NBA dataset and JPL Horizons dataset, with 11 and 12 interacting objects respectively. \model performs better than the baselines at short and long terms.}\label{tab:pred_mse_nba}
\vspace{-1.0em}
\end{wraptable}


==> graphics/table-nba.tex <==
\begin{wraptable}{r}{0.6\textwidth}
\centering
% \vspace{5.5em}
\vspace{-3em}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{\textbf{NBA SportsVU}}\\ \midrule
Prediction steps & 1 & 10 & 20 \\ \midrule
Static & 2.13e-4 & 3.04e-3 & 1.07e-2 \\
LSTM (joint) & 8.07e-5 & 1.42e-3 & 5.31e-3 \\
{Cond. GNN} & {1.71e-4} & {1.12e-3} & {3.11e-3} \\                        
NCI (Ours)  & \textbf{1.27e-5} & \textbf{3.46e-4} & \textbf{1.86e-3}\\
\bottomrule
\end{tabular}
\caption{\small Mean squared error (MSE) in predicting future states for NBA dataset with 11 interacting objects. \model performs better than the baseline at short and long terms.}\label{tab:pred_mse_nba}
\vspace{-1.0em}
\end{wraptable}


==> graphics/table_abl.tex <==
\begin{table*}[t!]
\centering
\vspace{-0.5em}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{\textbf{Charged}} \\ \midrule
Prediction steps & 1 & 10 & 20  \\ \midrule
\model  & 1.66e-5 & 1.64e-3 & 6.31e-3  \\
\bottomrule
\end{tabular}
\caption{\small Mean squared error (MSE) in predicting future states for simulations with 5 interacting objects.\\ \textbf{\model outperforms the baselines in mid to long-term prediction error}.}
\label{tab:pred_mse}
\vspace{-10pt}
\end{table*}

==> graphics/table_jhmdb.tex <==
% \begin{table}[t!]
% \small

\begin{wrapfigure}{R}{0.35\textwidth}
\centering
\vspace{-20pt}
\begin{tabular}{l|cc}
\toprule
& \multicolumn{2}{c}{\textbf{JHMDB}}  \\ \midrule
Prediction steps & 1 & 10  \\ \midrule
NRI & 6.71e-4	& 8.98e-3 \\
dNRI & 	&  \\
\model (Ours) & 3.05e-4 &	3.41e-3 \\
\bottomrule
\end{tabular}
% \vspace{-5pt}
\caption{\small \textbf{Mean squared error (MSE) in predicting future states for JHMDB dataset}, with 12 nodes for each limb joint. \model performs better than the baselines.}\label{tab:pred_mse_nba_jpl}
% \vspace{ -15pt}
\end{wrapfigure}


==> secs/checklist.tex <==
\section*{Checklist}
%%% BEGIN INSTRUCTIONS %%%

%%% END INSTRUCTIONS %%%
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} In the Appendix.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}
\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}
\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}. Code, data generation code and instructions will be released.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} Section \ref{sec:exp} contains some of this information. In the Appendix we discuss it in more depth.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} For some of the experiments.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? 
    \answerYes{} Added to the Appendix.
\end{enumerate}
\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}  
    \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}
\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
